A Trust-Region Algorithm for Noisy Equality Constrained Optimization

This paper introduces a modified Byrd-Omojokun (BO) trust region algorithm to address the challenges posed by noisy function and gradient evaluations. The original BO method was designed to solve equality constrained problems and it forms the backbone of some interior point methods for general large-scale constrained optimization. A key strength of the BO method is its robustness in handling problems with rank-deficient constraint Jacobians. The algorithm proposed in this paper introduces a new criterion for accepting a step and for updating the trust region that makes use of an estimate in the noise in the problem. The analysis presented here gives conditions under which the iterates converge to regions of stationary points of the problem, determined by the level of noise. This analysis is more complex than for line search methods because the trust region carries (noisy) information from previous iterates. Numerical tests illustrate the practical performance of the algorithm.

==> dump_aux_lemmas.tex <==
\begin{comment}


\begin{lemma}[Auxiliary Result]
Let the following be defined as:
\be 
\begin{split}
\phi &= \frac{ \mM \Delta_k^2 + \mE_1 \Delta_k + 2\mE_0}{\frac{\theta}2 \frac{\|y_k\|}{\|r_k\|} \min\left(\psi \Delta_k ,\frac{\|y_k\|}{\|B_k\|} \right) + \mu\mE_0 }
\end{split}
\ee
Where $\|B_k\| \leq \mM $, $\|r_k\|\leq L_r$, $\psi\in(0,1]$, $\theta\in(0,1]$, $\mu \geq 2$ are constants; 

Given any constant $\gamma>0$ such that
\be \|y_k\| > \frac{\mu}{\theta\psi} L_r  \mE_1 + \gamma \ee
and that 
\be \Delta_k < \bar\Delta := \frac{\theta\psi}{\mu \max(1,L_r) \mM}\gamma\ee
then
\be \phi < \frac{2}{\mu}.\ee
\end{lemma}

\begin{proof}


First note:
\be
\psi \Delta_k \leq \Delta_k < \frac{\theta\psi}{\mu \max(1,L_r) \mM}\gamma < \frac{\gamma}{\mM} < \frac{\|y_k\|}{\|B_k\|}
\ee
thus
\be \min\left(\psi \Delta_k ,\frac{\|y_k\|}{\|B_k\|} \right) = \psi \Delta_k.\ee
also note:
\be 
\begin{split}
\mM \Delta_k + \mE_1 
&< \mM \bar\Delta + \mE_1\\
& = \frac{\theta\psi}{\mu \max(1,L_r)}\gamma + \mE_1 \\
&< \frac{\theta\psi}{\mu L_r}\gamma + \mE_1\\
&= \frac{\theta \psi}{\mu L_r}\left[ {\gamma} + \frac{\mu}{\theta \psi}L_r \mE_1\right]\\
&<\frac{\theta \psi}{\mu L_r} \|y_k\|
\end{split}
\ee
Finally
\be 
\begin{split}
\phi &= \frac{ \mM \Delta_k^2 + \mE_1 \Delta_k + 2\mE_0}{\frac{\theta}2 \frac{\|y_k\|}{\|r_k\|} \min\left(\psi \Delta_k ,\frac{\|y_k\|}{\|B_k\|} \right) + \mu\mE_0 }\\
&= \frac{ \mM \Delta_k^2 + \mE_1 \Delta_k + 2\mE_0}{\frac{\theta\psi}2 \frac{\|y_k\|}{\|r_k\|}  \Delta_k + \mu\mE_0 }\\
&< \frac{ (\mM \Delta_k + \mE_1) \Delta_k + 2\mE_0}{\frac{\theta\psi}{2L_r} \|y_k\| \Delta_k + \mu\mE_0 }\\
&< \frac{ \frac{\theta \psi}{\mu L_r} \|y_k\| \Delta_k + 2\mE_0}{\frac{\theta\psi}{2L_r} \|y_k\| \Delta_k + \mu\mE_0 }\\
&= \frac{2}{\mu}
\end{split}
\ee

\end{proof}


\begin{lemma}[Auxiliary Result 2]
Let the following be defined as: 

\shig{spred: `some pred' }
\be 
\begin{split}
\rho &= \frac{\ared + 2\mE_0}{\spred + \mu\mE_0 }
\end{split}
\ee
If 
\be 
\begin{split}
\spred > \frac{\theta}2 \frac{\|y_k\|}{\|r_k\|} \min\left(\psi \Delta_k ,\frac{\|y_k\|}{\|B_k\|} \right)  
\end{split}
\ee
Where $\|B_k\| \leq \mM $, $\|r_k\|\leq L_r$, $\psi\in(0,1]$, $\theta\in(0,1]$, $\mu \geq 2$ are constants; 
Given constant $\eta$ , where 
\be\gamma = \frac\mu{2\theta\psi}\left[{-{\mE_1}  L_r + \sqrt{(\mE_1L_r)^2-8\tau[1 -2/(\mu c_0)]\max(1,L_r)\mM\mE_0}}\right] + \varepsilon\ee
\be  \|y_k\| >  \frac{\mu}{\psi\theta} L_r  \mE_1 + \gamma  \ee
and
\be \Delta_k >  \bar\Delta := \frac{\theta\psi}{\mu \max(1,L_r) \tau M}\gamma \ee
Then $\rho > c_0$ implies:
\be \ared > \ee
\end{lemma}


\begin{proof} 
First note that as $\bar \Delta < \gamma/\mM<\|y_k\| / \|B_k\|$:
\be \min\left(\psi \Delta_k ,\frac{\|y_k\|}{\|B_k\|} \right) > \min\left(\psi \bar\Delta ,\frac{\|y_k\|}{\|B_k\|} \right) \geq \psi\bar\Delta   \ee


Re-write $\rho > c_0$ as:
\be 
\begin{split}
\ared 
&> c_0 \spred + (c_0\mu -2)\mE_0\\
&>c_0\left[  \frac{\theta}2 \frac{\|y_k\|}{\|r_k\|} \min\left(\psi \Delta_k ,\frac{\|y_k\|}{\|B_k\|} \right)   \right] + (c_0\mu -2)\mE_0\\
&> \frac{c_0 \theta \psi }2  \frac{\|y_k\|}{\|r_k\|} \bar \Delta + (c_0\mu -2)\mE_0\\
&>  \frac{c_0 \theta \psi }2 \left(   	 \frac{\mu}{\psi\theta}   \mE_1 + \frac{\gamma}{L_r}	\right)\frac{\theta\psi}{\mu \max(1,L_r) \tau M}\gamma + (c_0\mu -2)\mE_0\\
&= \frac{c_0 (\theta \psi)^2 }{2\mu \max(1,L_r) \tau M} \left(   	 \frac{\mu}{\psi\theta}   \mE_1 + \frac{\gamma}{L_r}	\right)\gamma + (c_0\mu -2)\mE_0\\
&=\varepsilon\sqrt{\frac{c_0^2\theta\psi\mE_1^2}{4\max(1,L_r)^2\mM^2}+4 (2 - c_0\mu )\mE_0/L_r} + \frac{c_0 (\theta \psi)^2 }{2\mu L_r\max(1,L_r) \tau M} \varepsilon^2\\
&>\frac{c_0 (\theta \psi)^2 }{2\mu L_r\max(1,L_r) \tau M} \varepsilon^2
\end{split}
\ee
%\be\gamma = \frac12[-bc + \sqrt{b^2c^2-4e/a}] + \eta\ee




%\be\gamma = \frac12\left[{-\frac{\mu\mE_1}{\theta\psi}  L_r + \sqrt{(\frac{\mu\mE_1}{\psi\theta} )^2L_r^2-8\mu\tau\mM(\mu -2/c_0)\mE_0/[(\theta \psi)^2]}}\right] + \eta\ee




\be\gamma = \frac\mu{2\theta\psi}\left[{-{\mE_1}  L_r + \sqrt{(\mE_1L_r)^2-8\tau[1 -2/(\mu c_0)]\max(1,L_r)\mM\mE_0}}\right] + \varepsilon\ee



\end{proof}

\newpage

 \jn{[JN: not clear how much of the following is needed]}
 
 %\shig{[....moved here ....]}
 
 
 \shig{Before presenting the algorithm, we quickly remark one important property of the algorithm concerning the tangential step update, \st{which allows for re-writing the constrained subproblem into a unconstrained trust region subproblem to allow us to use existing theory and numerical techniques.}}
We may see this as a step aiming to improve optimality. We produce a `horizontal step' ($h_k$) which solves (substitute $p_k = v_k + h_k$ to the relaxed SQP and using $v_k\perp h_k$)
\begin{align}
\min_h\quad  &(\tg_{k}+\nabla_{x}^{2} \tW_k v_k)^{T} h+\frac{1}{2} h^{T} \nabla_{x}^{2} \tW_k h\\
 \text{ subject to }\quad &\|h \|\leq \sqrt{\Delta_k^2 - \|v_k\|^2}
\end{align}
%\shig{[be careful with $h_k$ must be in the null space of $\tA_k$ here, we must have that $\tZ_k$, spanning matrix of null of $\tA_k$ here somewhere. Just the two above equations are not enough:] (also check the choice of $Z_k$ here)}
\be h_k = \tZ_k d_k \quad \text{where}\quad \tZ_k = (I -\tA_k)^T\ee
We re-write the horizontal problem again here \shig{[Gilbert (2.28)]}:
{
\begin{align}\label{eq:hprob}
\min_d \quad  &(\tg_{k}+\nabla_{x}^{2} \tW_k v_k)^{T} \tZ_k d+\frac{1}{2} d^{T} \left[\tZ_k^T\nabla_{x}^{2} \tW_k \tZ_k\right] d\\
 \text{ subject to }\quad &\|\tZ_k d \|\leq \sqrt{\Delta_k^2 - \|v_k\|^2}
\end{align}

note here:
\be  \sqrt{\Delta_k^2 - \|v_k\|^2} \geq (1-\zeta)\Delta_k\ee
and the update for $p_k$ is
\be p_k = v_k +\tZ_k d_k\ee}

To summarize the subproblem, which was all that was discussed to this point, we generate, within each subproblem a step $v_k$ in the range of $\tA_k$ which improves feasibility and generate a step $u_k$ in the null space of $\tA_k$ which improves optimality. 
\shig{[ .... moved here .... ]}
 
  \jn{[JN: I left the following chunks. Do we need them?]}

%\shig{[check notation of this following]}
\be \Rightarrow \pred_k(p_k) =  -p_k^{T} \tg_{k}-\frac{1}{2} p_k^{T} \tW_{k} p_k + \nu_k  \vpred_k(p_k) \ee
Before the step acceptance test is imposed, we update the penalty parameter $\nu_k$ by requiring that it be large enough   such that


The accepted steps admits:
%\be \ared_k(p_k) = \tphi_k - \tphi_{k+1}>c_0\pred_k(p_k) > \pic_0 \nu_k\vpred_k(p_k)\ee
\be 
	\ared_k(p_k)  = \tphi(x_k,\nu_k)- \tphi(x_k+p_k,\nu_k) >  c_0 \pi \nu_k \vpred_k - (c_0 -1)\xi(\eps_f + \nu_{k} \eps_c).
\ee
Since $p_k  =v_k + h_k= v_k +\tZ_k d_k$, that $ \tA^T_k \tZ_k = 0$
\be \hpred_k(p_k) =-(\tg_{k}+\tW_k v_k)^{T} \tZ_k d_k-\frac{1}{2} d_k^{T} \left[\tZ_k^T \tW_k \tZ_k\right] d_k \ee 
\be = -(\tg_{k}+\tW_k v_k)^{T} h_k-\frac{1}{2} h_k^{T} \tW_k h_k \ee
\jn{[End of material the needs to be reorganized]}



\begin{lemma}[Cauchy Improvement in Feasibility by Horizontal Step]\shig{(Lemma 3, Gilbert)}
The improvement generated by the horizontal step perform at least as well as Cauchy step, it follows: 
\be \hpred_k(p_k) \geq \frac12 \left\|(\tilde g_{k}+\nabla_{x}^{2} L_k v_k)^{T} Z_k \right\| \min\left( \hat \Delta_k,  \frac{\|(\tilde g_{k}+\nabla_{x}^{2} L_k v_k)^{T} Z_k\|}{ \|Z_k^T\nabla_{x}^{2} L_k Z_k \|}\right)
%p_k-\frac{1}{2} p_k^{T} \left[Z_k^T\nabla_{x}^{2} L_k Z_k\right] p_k 
\ee 
\end{lemma}

\end{comment}



\shig{[Shigeng: Here I deleted two Auxilary Lemmas and kept in the dump file next to this main file. Can reference to the Tex Source File if Needed in the future.]}




\begin{lemma}[Auxiliary Result]
Let the following be defined as:
\be 
\begin{split}
\phi &= \frac{ \mM \Delta_k^2 + \mE_1 \Delta_k + 2\mE_0}{\frac{\theta}2 \frac{\|y_k\|}{\|r_k\|} \min\left(\psi \Delta_k ,\frac{\|y_k\|}{\|B_k\|} \right) + \mu\mE_0 }
\end{split}
\ee
Where $\|B_k\| \leq \mM $, $\|r_k\|\leq L_r$, $\psi\in(0,1]$, $\theta\in(0,1]$, $\mu \geq 2$ are constants; 

Given any constant $\gamma>0$ such that
\be \|y_k\| > \frac{\mu}{\theta\psi} L_r  \mE_1 + \gamma \ee
and that 
\be \Delta_k < \bar\Delta := \frac{\theta\psi}{\mu \max(1,L_r) \mM}\gamma\ee
then
\be \phi < \frac{2}{\mu}.\ee
\end{lemma}

\begin{proof}


First note:
\be
\psi \Delta_k \leq \Delta_k < \frac{\theta\psi}{\mu \max(1,L_r) \mM}\gamma < \frac{\gamma}{\mM} < \frac{\|y_k\|}{\|B_k\|}
\ee
thus
\be \min\left(\psi \Delta_k ,\frac{\|y_k\|}{\|B_k\|} \right) = \psi \Delta_k.\ee
also note:
\be 
\begin{split}
\mM \Delta_k + \mE_1 
&< \mM \bar\Delta + \mE_1\\
& = \frac{\theta\psi}{\mu \max(1,L_r)}\gamma + \mE_1 \\
&< \frac{\theta\psi}{\mu L_r}\gamma + \mE_1\\
&= \frac{\theta \psi}{\mu L_r}\left[ {\gamma} + \frac{\mu}{\theta \psi}L_r \mE_1\right]\\
&<\frac{\theta \psi}{\mu L_r} \|y_k\|
\end{split}
\ee
Finally
\be 
\begin{split}
\phi &= \frac{ \mM \Delta_k^2 + \mE_1 \Delta_k + 2\mE_0}{\frac{\theta}2 \frac{\|y_k\|}{\|r_k\|} \min\left(\psi \Delta_k ,\frac{\|y_k\|}{\|B_k\|} \right) + \mu\mE_0 }\\
&= \frac{ \mM \Delta_k^2 + \mE_1 \Delta_k + 2\mE_0}{\frac{\theta\psi}2 \frac{\|y_k\|}{\|r_k\|}  \Delta_k + \mu\mE_0 }\\
&< \frac{ (\mM \Delta_k + \mE_1) \Delta_k + 2\mE_0}{\frac{\theta\psi}{2L_r} \|y_k\| \Delta_k + \mu\mE_0 }\\
&< \frac{ \frac{\theta \psi}{\mu L_r} \|y_k\| \Delta_k + 2\mE_0}{\frac{\theta\psi}{2L_r} \|y_k\| \Delta_k + \mu\mE_0 }\\
&= \frac{2}{\mu}
\end{split}
\ee

\end{proof}


\begin{lemma}[Auxiliary Result 2]
Let the following be defined as: 

\shig{spred: `some pred' }
\be 
\begin{split}
\rho &= \frac{\ared + 2\mE_0}{\spred + \mu\mE_0 }
\end{split}
\ee
If 
\be 
\begin{split}
\spred > \frac{\theta}2 \frac{\|y_k\|}{\|r_k\|} \min\left(\psi \Delta_k ,\frac{\|y_k\|}{\|B_k\|} \right)  
\end{split}
\ee
Where $\|B_k\| \leq \mM $, $\|r_k\|\leq L_r$, $\psi\in(0,1]$, $\theta\in(0,1]$, $\mu \geq 2$ are constants; 
Given constant $\eta$ , where 
\be\gamma = \frac\mu{2\theta\psi}\left[{-{\mE_1}  L_r + \sqrt{(\mE_1L_r)^2-8\tau[1 -2/(\mu c_0)]\max(1,L_r)\mM\mE_0}}\right] + \varepsilon\ee
\be  \|y_k\| >  \frac{\mu}{\psi\theta} L_r  \mE_1 + \gamma  \ee
and
\be \Delta_k >  \bar\Delta := \frac{\theta\psi}{\mu \max(1,L_r) \tau M}\gamma \ee
Then $\rho > c_0$ implies:
\be \ared > \ee
\end{lemma}


\begin{proof} 
First note that as $\bar \Delta < \gamma/\mM<\|y_k\| / \|B_k\|$:
\be \min\left(\psi \Delta_k ,\frac{\|y_k\|}{\|B_k\|} \right) > \min\left(\psi \bar\Delta ,\frac{\|y_k\|}{\|B_k\|} \right) \geq \psi\bar\Delta   \ee


Re-write $\rho > c_0$ as:
\be 
\begin{split}
\ared 
&> c_0 \spred + (c_0\mu -2)\mE_0\\
&>c_0\left[  \frac{\theta}2 \frac{\|y_k\|}{\|r_k\|} \min\left(\psi \Delta_k ,\frac{\|y_k\|}{\|B_k\|} \right)   \right] + (c_0\mu -2)\mE_0\\
&> \frac{c_0 \theta \psi }2  \frac{\|y_k\|}{\|r_k\|} \bar \Delta + (c_0\mu -2)\mE_0\\
&>  \frac{c_0 \theta \psi }2 \left(   	 \frac{\mu}{\psi\theta}   \mE_1 + \frac{\gamma}{L_r}	\right)\frac{\theta\psi}{\mu \max(1,L_r) \tau M}\gamma + (c_0\mu -2)\mE_0\\
&= \frac{c_0 (\theta \psi)^2 }{2\mu \max(1,L_r) \tau M} \left(   	 \frac{\mu}{\psi\theta}   \mE_1 + \frac{\gamma}{L_r}	\right)\gamma + (c_0\mu -2)\mE_0\\
&=\varepsilon\sqrt{\frac{c_0^2\theta\psi\mE_1^2}{4\max(1,L_r)^2\mM^2}+4 (2 - c_0\mu )\mE_0/L_r} + \frac{c_0 (\theta \psi)^2 }{2\mu L_r\max(1,L_r) \tau M} \varepsilon^2\\
&>\frac{c_0 (\theta \psi)^2 }{2\mu L_r\max(1,L_r) \tau M} \varepsilon^2
\end{split}
\ee
%\be\gamma = \frac12[-bc + \sqrt{b^2c^2-4e/a}] + \eta\ee




%\be\gamma = \frac12\left[{-\frac{\mu\mE_1}{\theta\psi}  L_r + \sqrt{(\frac{\mu\mE_1}{\psi\theta} )^2L_r^2-8\mu\tau\mM(\mu -2/c_0)\mE_0/[(\theta \psi)^2]}}\right] + \eta\ee




\be\gamma = \frac\mu{2\theta\psi}\left[{-{\mE_1}  L_r + \sqrt{(\mE_1L_r)^2-8\tau[1 -2/(\mu c_0)]\max(1,L_r)\mM\mE_0}}\right] + \varepsilon\ee



\end{proof}

\newpage

 \jn{[JN: not clear how much of the following is needed]}
 
 %\shig{[....moved here ....]}
 
 
 \shig{Before presenting the algorithm, we quickly remark one important property of the algorithm concerning the tangential step update, \st{which allows for re-writing the constrained subproblem into a unconstrained trust region subproblem to allow us to use existing theory and numerical techniques.}}
We may see this as a step aiming to improve optimality. We produce a `horizontal step' ($h_k$) which solves (substitute $p_k = v_k + h_k$ to the relaxed SQP and using $v_k\perp h_k$)
\begin{align}
\min_h\quad  &(\tg_{k}+\nabla_{x}^{2} \tW_k v_k)^{T} h+\frac{1}{2} h^{T} \nabla_{x}^{2} \tW_k h\\
 \text{ subject to }\quad &\|h \|\leq \sqrt{\Delta_k^2 - \|v_k\|^2}
\end{align}
%\shig{[be careful with $h_k$ must be in the null space of $\tA_k$ here, we must have that $\tZ_k$, spanning matrix of null of $\tA_k$ here somewhere. Just the two above equations are not enough:] (also check the choice of $Z_k$ here)}
\be h_k = \tZ_k d_k \quad \text{where}\quad \tZ_k = (I -\tA_k)^T\ee
We re-write the horizontal problem again here \shig{[Gilbert (2.28)]}:
{
\begin{align}%\label{hprob}
\min_d \quad  &(\tg_{k}+\nabla_{x}^{2} \tW_k v_k)^{T} \tZ_k d+\frac{1}{2} d^{T} \left[\tZ_k^T\nabla_{x}^{2} \tW_k \tZ_k\right] d\\
 \text{ subject to }\quad &\|\tZ_k d \|\leq \sqrt{\Delta_k^2 - \|v_k\|^2}
\end{align}

note here:
\be  \sqrt{\Delta_k^2 - \|v_k\|^2} \geq (1-\zeta)\Delta_k\ee
and the update for $p_k$ is
\be p_k = v_k +\tZ_k d_k\ee}

To summarize the subproblem, which was all that was discussed to this point, we generate, within each subproblem a step $v_k$ in the range of $\tA_k$ which improves feasibility and generate a step $u_k$ in the null space of $\tA_k$ which improves optimality. 
\shig{[ .... moved here .... ]}
 
  \jn{[JN: I left the following chunks. Do we need them?]}

%\shig{[check notation of this following]}
\be \Rightarrow \pred_k(p_k) =  -p_k^{T} \tg_{k}-\frac{1}{2} p_k^{T} \tW_{k} p_k + \nu_k  \vpred_k(p_k) \ee
Before the step acceptance test is imposed, we update the penalty parameter $\nu_k$ by requiring that it be large enough   such that


The accepted steps admits:
%\be \ared_k(p_k) = \tphi_k - \tphi_{k+1}>c_0\pred_k(p_k) > \pic_0 \nu_k\vpred_k(p_k)\ee
\be 
	\ared_k(p_k)  = \tphi(x_k,\nu_k)- \tphi(x_k+p_k,\nu_k) >  c_0 \pi \nu_k \vpred_k - (c_0 -1)\xi(\eps_f + \nu_{k} \eps_c).
\ee
Since $p_k  =v_k + h_k= v_k +\tZ_k d_k$, that $ \tA^T_k \tZ_k = 0$
\be \hpred_k(p_k) =-(\tg_{k}+\tW_k v_k)^{T} \tZ_k d_k-\frac{1}{2} d_k^{T} \left[\tZ_k^T \tW_k \tZ_k\right] d_k \ee 
\be = -(\tg_{k}+\tW_k v_k)^{T} h_k-\frac{1}{2} h_k^{T} \tW_k h_k \ee
\jn{[End of material the needs to be reorganized]}



\begin{lemma}[Cauchy Improvement in Feasibility by Horizontal Step]\shig{(Lemma 3, Gilbert)}
The improvement generated by the horizontal step perform at least as well as Cauchy step, it follows: 
\be \hpred_k(p_k) \geq \frac12 \left\|(\tilde g_{k}+\nabla_{x}^{2} L_k v_k)^{T} Z_k \right\| \min\left( \hat \Delta_k,  \frac{\|(\tilde g_{k}+\nabla_{x}^{2} L_k v_k)^{T} Z_k\|}{ \|Z_k^T\nabla_{x}^{2} L_k Z_k \|}\right)
%p_k-\frac{1}{2} p_k^{T} \left[Z_k^T\nabla_{x}^{2} L_k Z_k\right] p_k 
\ee 
\end{lemma}
